FlowTS: Time Series Generation via Rectified Flow

Diffusion-based models have significant achievements in time series generation but suffer from inefficient computation: solving high-dimensional ODEs/SDEs via iterative numerical solvers demands hundreds to thousands of drift function evaluations per sample, incurring prohibitive costs. To resolve this, we propose FlowTS, an ODE-based model that leverages rectified flow with straight-line transport in probability space. By learning geodesic paths between distributions, FlowTS achieves computational efficiency through exact linear trajectory simulation, accelerating training and generation while improving performances. We further introduce an adaptive sampling strategy inspired by the exploration-exploitation trade-off, balancing noise adaptation and precision. Notably, FlowTS enables seamless adaptation from unconditional to conditional generation without retraining, ensuring efficient real-world deployment. Also, to enhance generation authenticity, FlowTS integrates trend and seasonality decomposition, attention registers (for global context aggregation), and Rotary Position Embedding (RoPE) (for position information). For unconditional setting, extensive experiments demonstrate that FlowTS achieves state-of-the-art performance, with context FID scores of 0.019 and 0.011 on Stock and ETTh datasets (prev. best: 0.067, 0.061). For conditional setting, we have achieved superior performance in solar forecasting (MSE 213, prev. best: 375) and MuJoCo imputation tasks (MSE 7e-5, prev. best 2.7e-4). The code is available at https://github.com/UNITES-Lab/FlowTS.

==> introduction-backup.tex <==
\section{Introduction}
Recent years have seen significant advancements in time series generation, including VAE-based approaches~\citep{desai2021timevaevariationalautoencodermultivariate,xu2020cotgangeneratingsequentialdata}, GAN-based methods, and diffusion-based techniques~\citep{kong2021diffwaveversatilediffusionmodel,tashiro2021csdi}. 
Among these, diffusion-based methods have demonstrated leading performance by explicitly modeling the iterative denoising process, enabling high-quality reconstructions. Despite these strengths, a critical limitation persists: \textit{inefficient computation}. 
Generating a single sample requires solving high-dimensional Ordinary/Stochastic Differential Equations (ODEs)/SDEs through iterative numerical solvers, necessitating hundreds to thousands of evaluations of the parameterized drift function, a prohibitive cost for real-world deployment. 
{Furthermore, optimizing these models demands extensive hyperparameter searches in complex design spaces \citep{karras2022elucidating}, complicating their adoption even in resource-rich settings.}

To address this limitation, we propose \textsc{FlowTS}, an ODE-based generative model designed for highly efficient time series generation. Unlike iterative denoising diffusion methods, \textsc{FlowTS} learns to transport the data distribution $\pi_0$ to the target $\pi_1$ via straight-line paths in the probability space. 
By bridging the gap between one-step and continuous-time models, \textsc{FlowTS} unifies two key advantages: 
\textit{i)} theoretical optimality through transport-cost-minimizing geodesics; 
\textit{(ii)} computational efficiency via exact simulation along straight trajectories, eliminating iterative steps.
This design accelerates both training and generation while reducing numerical error.
Furthermore, by employing straight-line paths and an unconstrained least-squares procedure for its rectified flow \citep{liu2022flow}, \textsc{FlowTS} avoids the instability issues common to GANs.
We also propose a simple yet highly effective adaptive sampling strategy, inspired by the exploration-exploitation trade-off \cite{sutton2018reinforcement}, which optimally balances an early focus on accommodating higher noise levels with a subsequent shift toward denser and more precise sampling.
Notably, \textsc{FlowTS}’s novel inference mechanism allows a model trained in unconditional settings to seamlessly adapt to conditional tasks without retraining.


Ensuring the authenticity of generated time series remains a key challenge. 
To address this, we incorporate trend and seasonality components to explicitly capture periodic and long-term patterns, following \citep{yuan2024diffusionts}.
However, such explicit decomposition often neglects unobserved global dependencies (e.g., latent interactions). 
To bridge this gap, we exploit attention register tokens\cite{darcet2023vision, }, a mechanism first pioneered in vision \cite{darcet2023vision}, which maintains persistent ``memory tokens'' that aggregate global context across series.
These registers capture and maintain global patterns, allowing the sequence tokens to concentrate on local temporal dependencies and ensuring holistic coherence.
Furthermore, we employ Rotary Position Embedding (RoPE) \cite{su2024roformer} to encode positional information via rotation matrices. 
RoPE offers two notable advantages: a natural decay property that aligns with real-world temporal dependencies and the ability to accommodate variable sequence lengths.
Together with attention registers, RoPE, and trend and seasonality components, \textsc{FlowTS} effectively captures both local and global dependencies, significantly enhancing the authenticity of generated time series.


We summarize our contributions:
\begin{itemize}
\vspace{-2mm}
    \item We introduce \textsc{FlowTS}, a pioneering approach that utilizes rectified flow with ODE-based straight-line transport for time series generation. This design achieves highly efficient generation, and an adaptive sampling strategy further balances exploration and exploitation for improved sample quality.
    \vspace{-1mm}
    \item We explicitly model global information and positional structure using attention register and RoPE, enhancing the authenticity of generated time series.
    \vspace{-1mm}
    \item \textsc{FlowTS} achieves state-of-the-art performance, {with context FID scores of \textit{{0.019}} and \textit{{0.011}} on Stock and ETTh datasets} (prev. best: 0.067, 0.061). {In solar forecasting, it lowers MSE to 213, a 43.2\% improvement over the previous best of 375}.

\end{itemize}



